Code Linting using Language Models

Code linters play a crucial role in developing high-quality software systems by detecting potential problems (e.g., memory leaks) in the source code of systems. Despite their benefits, code linters are often language-specific, focused on certain types of issues, and prone to false positives in the interest of speed. This paper investigates whether large language models can be used to develop a more versatile code linter. Such a linter is expected to be language-independent, cover a variety of issue types, and maintain high speed. To achieve this, we collected a large dataset of code snippets and their associated issues. We then selected a language model and trained two classifiers based on the collected datasets. The first is a binary classifier that detects if the code has issues, and the second is a multi-label classifier that identifies the types of issues. Through extensive experimental studies, we demonstrated that the developed large language model-based linter can achieve an accuracy of 84.9% for the binary classifier and 83.6% for the multi-label classifier.

==> figures/unseenTypesDatasetPseudocode.tex <==
\begin{algorithm}
\small
\caption{Creating Datasets for Evaluating the Binary Classification Model on Identifying Unseen Issue Types}
\label{fig:unseenIssueDataset}
\begin{algorithmic}[1]
    \State mainDataset $\gets$ allTargetMethods()
    \State unseenIssueTypes $\gets$ \{\}
    \State testDataset $\gets$ \{\}
    \While{testDataset.size $< 0.05 *$ mainDataset.size} 
        \State selectedType $\gets$ randomIssueTypeFrom(mainDataset)
        \While{numTargetMethodsWithType(selectedType) $\geq 0.05 *$ mainDataset.size}
            \State selectedType $\gets$ randomIssueTypeFrom(mainDataset)
        \EndWhile
        \State unseenIssueTypes.add(selectedType)
        \For{method $in$ mainDataset}
            \If{method.issueTypes $\subseteq$ unseenIssueTypes}
                \State testDataset.add(method)
                \State mainDataset.remove(method)
            \EndIf
        \EndFor
    \EndWhile
    \For{method $in$ mainDataset}
        \If{(method.issueTypes $\cap$ unseenIssueTypes $\neq \{\}$)}
            \State mainDataset.remove(method)
        \EndIf
    \EndFor
    \For{$i \gets 0$ to testDataset.size}
        \State method $\gets$ randomMethodWithoutIssuesFrom(mainDataset)
        \State testDataset.add(method)
        \State mainDataset.remove(method)
    \EndFor
    \State trainDataset $\gets$ trainSplit(mainDataset)
    \State validationDataset $\gets$ validationSplit(mainDataset)
    \State baselineTestDataset $\gets$ testSplit(mainDataset)
   % \end{algorithmic}
    
  %  \caption{Algorithm for Creating Datasets for Evaluating the Binary Classification Model on Identifying Unseen Issue Types}
  %  
\end{algorithmic}
\end{algorithm}

==> tables/rq1-timeCompare.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{p{2.5cm} c c c c}
        \toprule
        \multirow{2}{3cm}{Case} & \multicolumn{4}{c}{Elapsed Time (Seconds)} \\
        & Min. & Max. & Mean & Std. Deviation \\
        \midrule
        Infer & 5.386 & 847.09 & 42.966 & 95.756 \\
        Java Extract & 1.247 & 23.751 & 4.514 & 4.006 \\
        Binary Model & 0.130 & 148.579 & 9.315 & 18.339 \\
        Multi-Label Model & 0.103 & 147.865 & 9.330 & 18.306 \\
        \midrule
        SpotBugs & 3.589 & 704.928 & 25.326 & 68.037 \\
        Java Extract & 0.322 & 47.015 & 3.962 & 4.988 \\
        Binary Model & 0.027 & 144.124 & 7.935 & 17.819 \\
        Multi-Label Model & 0.029 & 149.013 & 8.135 & 18.272 \\
        \bottomrule
    \end{tabular}
    \caption{The Elapsed Time in Seconds Comparing Both the Binary and Multi-Label Classification Models to the Infer and SpotBugs}
    \label{table:lintingElapsedTimes}
\end{table}

==> tables/rq3-1-binaryClassUnseenIssueTypes.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{l c c c c}
        \toprule
        Test Set Contents & Accuracy & Precision & Recall & F1 \\
        \midrule
        Seen Issue Types & 0.881 & 0.867 & 0.901 & 0.884 \\
        Unseen Issue Types & 0.570 & 0.671 & 0.275 & 0.390 \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of Binary Classification Performance on Test Sets Containing Issues Containing Either Seen or Unseen Issue types}
    \label{table:bcUnseenTypes}
\end{table}
